SPARTUN3D: Situated Spatial Understanding of 3D World in Large Language Models

Integrating the 3D world into large language models (3D-based LLMs) has been a promising research direction for 3D scene understanding. However, current 3D-based LLMs fall short in situated understanding due to two key limitations: 1) existing 3D datasets are constructed from a global perspective of the 3D scenes and lack situated context. 2) the architectures of existing 3D-based LLMs lack explicit alignment between the spatial representations of 3D scenes and natural language, limiting their performance in tasks requiring precise spatial reasoning. We address these issues by introducing a scalable situated 3D dataset, named Spartun3D, that incorporates various situated spatial reasoning tasks. Furthermore, we propose Spartun3D-LLM, built on an existing 3D-based LLM but integrated with a novel situated spatial alignment module, aiming to enhance the alignment between 3D visual representations and their corresponding textual descriptions. Experimental results demonstrate that both our proposed dataset and alignment module significantly enhance the situated spatial understanding of 3D-based LLMs.

==> sections/other.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
      \toprule[1.5pt]
       \textbf{Models} &  \multicolumn{5}{c}{\textbf{Situated Captioning}} &\multicolumn{5}{c}{\textbf{Attributes and Relations}} & \multicolumn{5}{c}{\textbf{Affordance}} & \multicolumn{5}{c}{\textbf{Situated Planning}}\\
        \cmidrule(lr){1-1} \cmidrule(lr){2-6} \cmidrule(lr){7-11}
        \cmidrule(lr){12-16} \cmidrule(lr){17-21}
         & C & B-4 & M & R & S & C & B-4 & M & R & EM & C & B-4 & M & R & S & C & B-4 & M & R & S\\
         \cmidrule(lr){1-21}
        % & $12.0$ & $0.08$ & $0.20$ & $0.25$ & $0.68$ \\
     % LEO+SiSU3D & $10.3$ & $0.13$ & $0.23$ &  $0.30$ & $0.73$\\
     
     LEO-Opt1.3B\\
     
     \hline
     LEO-Vicuna7B~(zero-shot) & $0.00$ & $0.00$ & $0.09$ & $0.15$ & $0.52$ & 1.00 & 0.00 & 0.17 & 0.39 & 0.43 & 0.13 & 0.00 & 0.03 & 0.05& 0.32& $0.00$ & $0.00$ & $0.07$ & $0.15$ & $59.2\%$\\
     Spartun3D-LLM(w/o align) & $1.47$ & $0.17$ & $0.23$ & $0.32$ & $0.76$ & $1.29$ &$0.10$ & $0.23$& $0.48$ & $0.53$
     % $1.37$ & $0.11$ & $0.24$ & $0.51$ & $0.57$ 
     & $2.11$ & $\mathbf{0.33}$ & $0.25$ & $0.55$ & $0.68$ & $2.47$ & $0.48$ & $0.36$ & $0.65$ & $85.8\%$\\
     Spartun3D(w/ align) & $\mathbf{1.47}$ & $\mathbf{0.19}$ & $\mathbf{0.23}$ & $\mathbf{0.33}$ & $\mathbf{0.78}$ & $1.35$ & $0.10$ & $0.25$ & $0.51$ & $0.56$ & $\mathbf{2.53}$ & $\mathbf{0.33}$ & $\mathbf{0.27}$ & $\mathbf{0.57}$ & $\mathbf{0.70}$ & \mathbf{2.52} & 0.48 & 0.36 & $\mathbf{0.66}$ & $\mathbf{88.7\%}$
     % $1.26$ & $0.18$ & $0.22$ & $0.47$ & $0.44$
     \\
      % LEO+SiSU3D & $114.05$ & $0.13$ & $0.20$ &  $0.43$ & $0.39 (0.45)$\\
    \bottomrule[1.5pt]
    \end{tabular}
    }
    \caption{Experimental Results on Spartun3D Tasks.\lifu{also show the zero-shot and fine-tuning results of other baselines}}
    \label{tab:Spartun3D results}
\end{table*}




\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}
    {c c c c c c c c c c c c c c c c c}
      \toprule[1.5pt]
       \multirow{2}{*}{\large{\textbf{LLMs}}} &    \multirow{2}{*}{\large{\textbf{Models}}} &\multicolumn{5}{c}{\textbf{Attributes and Relations}} & \multicolumn{5}{c}{\textbf{Affordance}} & \multicolumn{5}{c}{\textbf{Situated Planning}}\\
        \cmidrule(lr){3-7} \cmidrule(lr){8-12}
        \cmidrule(lr){13-17}
        & & C & B-4 & M & R & EM@1 & C & B-4 & M & R & S & C & B-4 & M & R & S\\
        \cmidrule(lr){1-17}
        % & $12.0$ & $0.08$ & $0.20$ & $0.25$ & $0.68$ \\
     % LEO+SiSU3D & $10.3$ & $0.13$ & $0.23$ &  $0.30$ & $0.73$\\
     \multirow{2}{*}{OPT1.3B} & LEO+Spartun3D & $121.3$ & $7.0$ & $20.1$ & $45.3$ & $47.7$ & 224.6 & 30.6 & 24.9 & 53.2 & 66.9 & 229.7 & 44.8 & 32.1 & 60.9 & 83.8\\
     & \rowcolor{cell_grey} Spartun3D-LLM & $124.1$ & $9.2$ & $21.0$ & $47.3$ & $49.4$ & $227.2$ & $31.4$ & $26.3$ & $54.1$ & $68.2$ & $232.3$ & $45.2$ & $33.2$ & $62.1$ & $85.4$ \\
     \cmidrule(lr){1-17} 
     \multirow{2}{*}{Vicuna7B} & LEO+Spartun3D  &  $125.4$ & $10.1$ & $22.1$ & $46.7$ & $52.1$ & $238.9$ & $32.1$ & $24.4$ & $55.0$ & $68.3$ & $242.1$ &  $46.5$ & $35.2$ & $63.1$ & $84.3$  \\
     & \rowcolor{cell_grey} Spartun3D-LLM & $131.2$ & $10.3$ & $24.3$ & $48.8$ &  $53.7$ & $240.4$ & $32.1$ & $25.0$ & $55.3$ & $68.7$ & $244.0$ & $47.1$ & $36.4$ & $64.0$ & $86.8$ \\
      \cmidrule(lr){1-17}
      \cmidrule(lr){1-17}  
     \multirow{3}{*}{Vicuna7B$^*$}& LEO~(zero-shot) &  $100.3$ & $0.00$ & $17.4$ & $39.1$ & $42.7$ & $13.3$ & $0.00$ & $3.00$ & $5.00$ & $32.3$ & $0.00$ & $0.00$ & $7.00$ & $15.3$ & $59.2$\\
     & LEO+Spartun3D & $129.2$ &$10.4$ & $23.0$& $48.1$ & $53.2$
     & $211.3$ & $\mathbf{32.1}$ & $24.6$ & $55.0$ & $67.8$ & $247.1$ & $47.5$ & $36.2$ & $65.1$ & $85.8$\\
    &\rowcolor{cell_grey} Spartun3D-LLM & $\mathbf{135.4}$ & $10.7$ & $24.9$ & $51.3$ & $\mathbf{56.9}$ & $\mathbf{254.7}$ & $\mathbf{32.9}$ & $\mathbf{26.7}$ & $\mathbf{57.3}$ & $\mathbf{69.7}$ & $\mathbf{252.1}$ & $47.6$ & $36.2$ & $\mathbf{65.4}$ & $\mathbf{88.7}$
     % $1.26$ & $0.18$ & $0.22$ & $0.47$ & $0.44$
     \\
      % LEO+SiSU3D & $114.05$ & $0.13$ & $0.20$ &  $0.43$ & $0.39 (0.45)$\\
    \bottomrule[1.5pt]
    \end{tabular}
    }
    \caption{Experimental Results on Spartun3D Situated QA Tasks. $*$ represents the model initialized with LEO pre-trained weights.
    [Keys: C: CIDER; B-4: BLEU-4; M: METEOR; R: ROUGE; Sim: sentence similarity; EM: top-1 exact match; Bold: best results].}
    \label{tab:qa results}
    \vspace{-3mm}
\end{table*}




\begin{wraptable}{r}{0.55\textwidth} 
    \centering
    \resizebox{0.55\textwidth}{!}{
    \begin{tabular}{c c c c c c c}
    \toprule[1pt]
       \textbf{LLMs} & & C & B-4 & M & R & S  \\
     \cmidrule(lr){1-7} 
       \multirow{2}{*}{Opt1.3B} & LEO+Spartun3D  & 5.9 & 15.3 & 17.7 & 31.2 & 67.3\\
       & \rowcolor{cell_grey} Spartun3D-LLM  & $6.4$ & $15.7$ & $18.5$ & $31.2$ & $68.6$\\ 
       \cmidrule(lr){1-7} 
        \multirow{2}{*}{Vicuna7B} & LEO+Spartun3D & 6.7 & 15.8 & 18.7 & 32.3 & 70.4\\
       & \rowcolor{cell_grey} Spartun3D-LLM  & $8.5$ & $16.4$ & $19.6$ & $32.5$ & $72.5$  \\ 
       \cmidrule(lr){1-7} 
       \multirow{3}{*}{Vicuna7B$^*$} & LEO~(zero-shot)  & $0.00$ & $0.00$ & $9.00$ & $15.3$ & $51.9$ \\
      & LEO+Spartun3D & $14.6$ & $17.2$ & $22.6$ & $32.1$ & $76.3$ \\
       & \rowcolor{cell_grey} Spartun3D-LLM  & $\mathbf{14.6}$ & $\mathbf{19.3}$ & $\mathbf{23.3}$ & $\mathbf{33.4}$ & $\mathbf{78.1}$ \\
    \bottomrule[1pt]
    \end{tabular}
    }
    \caption{Experimental Results on Spartun3D Situated Captioning Task.}
    \label{spartun3d caption}
\end{wraptable}
